Quantum capacity analysis of finite-dimensional lossy channels

Traditionally, Quantum Information, and Quantum Communication specifically, have been focused on qubit-based architectures. Recent results, however, highlighted that higher dimensional architectures (qudit-based) may present advantages both in terms of communication and computation; a family of channels called Multi-level Amplitude Damping (MAD) channels, which are a possible qudit generalization of the well known Amplitude Damping Channels, is able to model energy decay processes that may happen during signal transmission. In this work, the Quantum Capacity of 4-dimensional MAD's is studied, relying on a technique for computing it even outside of degradable and antidegradable conditions. We also characterized the complete region of antidegradability and degradability in the parameter space for a generic d-dimensional MAD using both analytical and semi-numerical methods.

==> figures/example/3Bschemealtcomplete.tex <==
\begin{tikzpicture}[scale=2.5]
	% Transition from 1
	\draw[black, thick] (2.2,0) -- (0.7,0) node [left] {\small{$\ket{0}$}};
	\draw[black, thick] (2.2,0.3) -- (0.7,0.3) node [left] {\small{$\ket{1}$}};
	\draw[black, thick] (2.2,0.6) -- (0.7,0.6) node [left] {\small{$\ket{2}$}};
	\draw[black, thick] (2.2,0.9) -- (0.7,0.9) node [left] {\small{$\ket{3}$}};
	\draw[MyGold, thick, ->] (1,0.6) -- (1,0.3) node [above left] {\footnotesize{$\gamma_{32}$}};
	\draw[MyGold, thick, ->] (1.3,0.6) -- (1.3,0) node [above left] {\footnotesize{$\gamma_{30}$}};
	\draw[MyGold, thick, ->] (1.9,0.9) -- (1.9,0) node [above left] {\footnotesize{$\gamma_{10}$}};
	\node[ellipse, minimum width = 1.5cm, minimum height = 3cm, draw=MyBlue, thick] at (1.9,0.45) (ellipse) {};
	\node[text=MyBlue] (tex) [below= 0.1 of ellipse.south] {$1-\gamma_{11}$};
\end{tikzpicture}

==> figures/example/3Bschemecomplete3.tex <==
\begin{tikzpicture}[scale=2.5]
	% Transition from 1
	\draw[black, thick] (2.2,0) -- (0.7,0) node [left] {\small{$\ket{0}$}};
	\draw[black, thick] (2.2,0.3) -- (0.7,0.3) node [left] {\small{$\ket{1}$}};
	\draw[black, thick] (2.2,0.6) -- (0.7,0.6) node [left] {\small{$\ket{2}$}};
	\draw[black, thick] (2.2,0.9) -- (0.7,0.9) node [left] {\small{$\ket{3}$}};
	\draw[MyGold, thick, ->] (1,0.3) -- (1,0) node [above left] {\footnotesize{$\gamma_{10}$}};
	\draw[MyGold, thick, ->] (1.6,0.9) -- (1.6,0.6) node [above left] {\footnotesize{$\gamma_{32}$}};
	\draw[MyGold, thick, ->] (1.9,0.9) -- (1.9,0) node [above left] {\footnotesize{$\gamma_{30}$}};
	\node[ellipse, minimum width = 2.1cm, minimum height = 3cm, draw=MyBlue, thick] at (1.75,0.45) (ellipse) {};
	\node[text=MyBlue] (tex) [below= 0.1 of ellipse.south] {$1-\gamma_{33}$};
\end{tikzpicture}

==> figures/example/3Btotal.tex <==
\begin{tikzpicture}
    \begin{axis}[
        view={55}{30}, % Roughly matches ViewPoint -> {0.7, 1, 1}
        width=12cm,
        height=12cm,
        xmin=0, xmax=1.1,
        ymin=0, ymax=1.1,
        zmin=0, zmax=1.1,
        xlabel={$\gamma_{32}$},
        ylabel={$\gamma_{30}$},
        zlabel={$\gamma_{10}$},
        axis lines=center,
        grid=major,
        % --- New Tick Definitions ---
        xtick={0, 0.5, 1},
        ytick={0, 0.5, 1},
        ztick={0, 0.5, 1},
        % ----------------------------
        xlabel style={anchor=west, font=\Large},
        ylabel style={anchor=west, font=\Large},
        zlabel style={anchor=south, font=\Large},
        tick label style={font=\normalsize}
    ]
    
    % Define styles based on PlotStyle and MeshStyle parameters
    \tikzset{
        blue face/.style={fill=blue, fill opacity=0.5, draw=gray, draw opacity=0.3, thin},
        red face/.style={fill=purple, fill opacity=0.3, draw=black, draw opacity=0.3, thin},
        yellow face/.style={fill=yellow, fill opacity=0.5, draw=black, draw opacity=0.3, thin},
        green face/.style={fill=green, fill opacity=0.5, draw=black, draw opacity=0.3, thin}
    }
    
    % =================================================================
    % DRAWING ORDER: Back to Front to handle opacity properly
    % =================================================================
    
    % 1. BLOCK 1 (degreg - Blue)
    \filldraw[blue face] (0,0,0) -- (0,0,0.5) -- (0.5,0,0.5) -- (0.5,0,0) -- cycle; % Bottom
    \filldraw[blue face] (0,0,0) -- (0,0,0.5) -- (0,0.5,0.5) -- (0,0.5,0) -- cycle; % Back
    \filldraw[blue face] (0,0,0) -- (0.5,0,0) -- (0,0.5,0) -- cycle; % Left
    \filldraw[blue face] (0,0,0.5) -- (0.5,0,0.5) -- (0,0.5,0.5) -- cycle; % Right
    \filldraw[blue face] (0.5,0,0) -- (0.5,0,0.5) -- (0,0.5,0.5) -- (0,0.5,0) -- cycle; % Slant
    
    % 2. BLOCK 2 (ND1 outer part - Red)
    \filldraw[red face] (0.5,0,0) -- (0.5,0,0.5) -- (1,0,0.5) -- (1,0,0) -- cycle; % Bottom-ish
    \filldraw[red face] (0,0.5,0) -- (0,0.5,0.5) -- (0,1,0.5) -- (0,1,0) -- cycle; % Back-ish
    \filldraw[red face] (0.5,0,0) -- (1,0,0) -- (0,1,0) -- (0,0.5,0) -- cycle; % Left
    \filldraw[red face] (0.5,0,0.5) -- (1,0,0.5) -- (0,1,0.5) -- (0,0.5,0.5) -- cycle; % Right
    \filldraw[red face] (0.5,0,0) -- (0.5,0,0.5) -- (0,0.5,0.5) -- (0,0.5,0) -- cycle; % Inner Slant
    \filldraw[red face] (1,0,0) -- (1,0,0.5) -- (0,1,0.5) -- (0,1,0) -- cycle; % Outer Slant
    
    % 3. BLOCK 3 (ND2 - Yellow)
    \filldraw[yellow face] (0,0,0.5) -- (0,0,1) -- (0.5,0,1) -- (0.5,0,0.5) -- cycle; % Bottom
    \filldraw[yellow face] (0,0,0.5) -- (0,0,1) -- (0,0.5,1) -- (0,0.5,0.5) -- cycle; % Back
    \filldraw[yellow face] (0,0,0.5) -- (0.5,0,0.5) -- (0,0.5,0.5) -- cycle; % Left
    \filldraw[yellow face] (0,0,1) -- (0.5,0,1) -- (0,0.5,1) -- cycle; % Right
    \filldraw[yellow face] (0.5,0,0.5) -- (0.5,0,1) -- (0,0.5,1) -- (0,0.5,0.5) -- cycle; % Slant
    
    % 4. BLOCK 4 (ND3 - Green)
    \filldraw[green face] (0.5,0,0.5) -- (0.5,0,1) -- (1,0,1) -- (1,0,0.5) -- cycle; % Bottom-ish
    \filldraw[green face] (0,0.5,0.5) -- (0,0.5,1) -- (0,1,1) -- (0,1,0.5) -- cycle; % Back-ish
    \filldraw[green face] (0.5,0,0.5) -- (1,0,0.5) -- (0,1,0.5) -- (0,0.5,0.5) -- cycle; % Left
    \filldraw[green face] (0.5,0,1) -- (1,0,1) -- (0,1,1) -- (0,0.5,1) -- cycle; % Right
    \filldraw[green face] (0.5,0,0.5) -- (0.5,0,1) -- (0,0.5,1) -- (0,0.5,0.5) -- cycle; % Inner Slant
    \filldraw[green face] (1,0,0.5) -- (1,0,1) -- (0,1,1) -- (0,1,0.5) -- cycle; % Outer Slant
    
    % =================================================================
    % RED DASHED LINES (drawn on top)
    % =================================================================
    \draw[red, thick, dashed] (0, 0, 0.5) -- (0, 1, 0.5);
    \draw[red, thick, dashed] (0, 0.5, 0) -- (0, 0.5, 1);
    \draw[red, thick, dashed] (1, 0, 0.5) -- (0, 0, 0.5);
    \draw[red, thick, dashed] (0.5, 0, 0) -- (0.5, 0, 1);
    \draw[red, thick, dashed] (0.5, 0, 0) -- (0, 0.5, 0);
    \draw[red, thick, dashed] (0.5, 0, 0.5) -- (0, 0.5, 0.5);
    
    \end{axis}
    \end{tikzpicture}
